Discretionary Trees: Understanding Street-Level Bureaucracy via Machine Learning

Street-level bureaucrats interact directly with people on behalf of government agencies to perform a wide range of functions, including, for example, administering social services and policing. A key feature of street-level bureaucracy is that the civil servants, while tasked with implementing agency policy, are also granted significant discretion in how they choose to apply that policy in individual cases. Using that discretion could be beneficial, as it allows for exceptions to policies based on human interactions and evaluations, but it could also allow biases and inequities to seep into important domains of societal resource allocation. In this paper, we use machine learning techniques to understand street-level bureaucrats' behavior. We leverage a rich dataset that combines demographic and other information on households with information on which homelessness interventions they were assigned during a period when assignments were not formulaic. We find that caseworker decisions in this time are highly predictable overall, and some, but not all of this predictivity can be captured by simple decision rules. We theorize that the decisions not captured by the simple decision rules can be considered applications of caseworker discretion. These discretionary decisions are far from random in both the characteristics of such households and in terms of the outcomes of the decisions. Caseworkers typically only apply discretion to households that would be considered less vulnerable. When they do apply discretion to assign households to more intensive interventions, the marginal benefits to those households are significantly higher than would be expected if the households were chosen at random; there is no similar reduction in marginal benefit to households that are discretionarily allocated less intensive interventions, suggesting that caseworkers are improving outcomes using their knowledge.

==> author_response.tex <==
\section{Author Response}
We appreciate the time and expertise of the reviewers and are grateful for their feedback. Here we address some of the thematic concerns raised by the reviews.

\textcolor{blue}{R4: Setting, motivation, justification} 
We are afraid that the reviewer might have misunderstood the motivation and setting of our research (the other reviewers have read the paper in line with our intentions). We would like to take this opportunity to clarify. Lipsky's theory of how street-level bureaucrats operate predicts that they would try and make decisions quickly on a majority of cases, using heuristics or simple rules, reserving their full cognitive power for more complex cases. Most prior work has been qualitative. We leverage a unique dataset and modern AI techniques to bring a quantitative lens to bear on the \emph{scientific question of how caseworkers behave.} A priori, it would have been entirely possible to find that there was no simple way to explain a majority of caseworker decisions! We instead find quantitative evidence in the data to affirm Lipsky's theory. This is itself a contribution (this kind of ``revealed preference'' approach  complements qualitative interviews which would ask caseworkers what they thought they were doing, which we know can be different from what they are actually doing).

A second question is about how caseworkers use their discretion. Two hypotheses suggested by Elster's theory of local justice (and pointed out as important questions for AI in Social Services by Das in a AAAI 2022 Blue Sky paper) is that they could be using their discretion to prioritize the most vulnerable or those who would benefit most. Our work provides evidence for the latter.

In terms of potential uses, we are certainly not suggesting replacement of human decision-makers. While we think the (social) scientific questions we consider are themselves important, our results can also inform the development of AI support tools for caseworkers -- without understanding what caseworkers do it is hard to even begin to think about the design of support tools, plus AI cannot be evaluated without considering the ``bureaucratic counterfactual'' described by Johnson and Zhang in FAccT 2022.

Finally, it is generally acknowledged that consistency in decision-making is important for a decision process to be accepted as procedurally fair, so the fact that we find such consistency is a positive in terms of the evaluation of past caseworker decision-making. 

\textcolor{blue}{R4: ``authors make no reference to the data-set they are working with.''}
We are puzzled by this assertion since the other reviewers mention our description of the data as a strength. We describe the data in the ``Backgrounds and Related Work'' section within the subsections ``The Data'' and ``Data Cleaning'' on page 3 of the submission. 

\textcolor{blue}{R1, R4: Confidence intervals for AUCs} Thank you for the suggestion. We calculated the confidence intervals of the AUC curves using DeLong's method and report these intervals in Table \ref{table:CI}. The confidence intervals are relatively tight and do not change the interpretation in any way. We will include these intervals in the final version.



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|ll|cc|}
\hline
\multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\textbf{SER-DT}} & \multicolumn{2}{c|}{\textbf{XGBoost}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Intervention Type}} & \multicolumn{1}{l|}{\textbf{AUC Value}} & \textbf{95\% AUC CI} & \multicolumn{1}{c|}{\textbf{AUC Value}} & \textbf{95\% AUC CI} \\ \hline
\textbf{Emergency Shelter} & \multicolumn{1}{l|}{0.7671} & {[}0.7452, 0.7890{]} & \multicolumn{1}{c|}{0.9452} & {[}0.9392, 0.9513{]} \\ \hline
\textbf{Transitional Housing} & \multicolumn{1}{l|}{0.8766} & {[}0.8547,0.8984{]} & \multicolumn{1}{c|}{0.9434} & {[}0.9360, 0.9507{]} \\ \hline
\textbf{Rapid Re-Housing} & \multicolumn{1}{l|}{0.7802} & {[}0.74634, 0.8170{]} & \multicolumn{1}{c|}{0.9299} & {[}0.9136, 0.9462{]} \\ \hline
\textbf{Prevention} & \multicolumn{1}{l|}{0.9480} & {[}0.9371, 0.9589{]} & \multicolumn{1}{c|}{0.9875} & {[}0.9846, 0.9904{]} \\ \hline
\end{tabular}%
}
\caption{95\% Confidence intervals for SER-DT (Sample size: 1907) and XGBoost (Sample size: 4239)}.
\label{table:CI}
\end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Intervention Type}} & \textbf{AUC Value} & \textbf{95\% AUC CI} \\ \hline
% \textbf{Emergency Shelter} & 0.7671 & {[}0.7452, 0.7890{]} \\ \hline
% \textbf{Transitional Housing} & 0.8766 & {[}0.8547, 0.8984{]} \\ \hline
% \textbf{Rapid Re-Housing} & 0.7802 & {[}0.7434, 0.8170{]} \\ \hline
% \textbf{Prevention} & 0.9480 & {[}0.9371, 0.9589{]} \\ \hline
% \end{tabular}
% \caption{95\% Confidence intervals for SER-DT. Sample size: 1907 }
% \label{table:CI}
% \end{table}

% CI for XGBoost 
% \begin{table}[]
% \centering
% \begin{tabular}{|l|c|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Intervention Type}} & \textbf{AUC Value} & \textbf{95\% AUC CI} \\ \hline
% \textbf{Emergency Shelter} & 0.9452 & {[}0.9392, 0.9513{]} \\ \hline
% \textbf{Transitional Housing} & 0.9434 & {[}0.9360, 0.9507{]} \\ \hline
% \textbf{Rapid Re-Housing} & 0.9299 & {[}0.9136, 0.9462{]} \\ \hline
% \textbf{Prevention} & 0.9875 & {[}0.9846, 0.9904{]} \\ \hline
% \end{tabular}
% \caption{95\% Confidence intervals for XGBoost. Sample size: 4239 }
% \end{table}

\textcolor{blue}{R1, R4: Unobserved confounding}
This is a fundamental and important issue, and we agree with the reviewers that unobserved confounding can always be an issue. It is entirely possible that caseworkers are picking up on cues through their (brief) interactions with the households, however, the fact that we achieve high AUCs using only observables does alleviate this concern somewhat, as suggested by R1. We would be excited by future work that uses advanced causal inference techniques to study such questions, but the applicability of such techniques is typically highly dependent on the setting.

\textcolor{blue}{R1, R3, and R4: SER-DT models versus others} 
We feel this question is well-captured by R1's version ``It seems likely that there could be many simple decision trees that have similar predictive accuracy. Have the authors studied this, and is there any way to show that a simple description of human decisions is well-identified?'' This is a great question, and this framing helps us sharpen our argument. First, short trees function the same as simple rules or the common understanding of heuristics in the behavioral sciences, which are typically contrasted with more cognitively demanding linear models (e.g. Hogarth and Karelaia in Psychological Review 2007). Second, among (short) tree learners, SER-DT, a relatively recent algorithm (NEurIPS 2022), stands out as its performance (AUC) is on par with models like CART while it performs much better on explainability metrics. 

Now, one can turn to asking about differences in predictive models that could be learned by SER-DT considering training set variation. It is important to note that the key question is about the implications of any model differences on the population they predict would receive different interventions. To test this, we compute rank correlations on ten different SER-DT models, demonstrating a high degree of similarity in the outputs of different models for both TH and ES, affirming consistency in model predictions and alleviating concerns about differences in tree outcomes.
\includegraphics[width=\columnwidth]{figs/correlations.png}

    %\caption{Spearman's Rank Correlation test for the 10 models we had for TH (left) and ES (right). We took predictions from the model with the highest test accuracy, but as we can see from this figure, there is a very high correlation between the predictions generated by the models, suggesting that the predictions generated by SER-DT are consistent across models, alleviating concerns of predictions being different across different models. }
    %\label{fig:rank_correlations}
%\end{figure}

%The SER-DT algorithm was featured in the proceedings of NeurIPS 2022. The authors conducted a comprehensive experimental evaluation of SER-DT's performance compared to the CART algorithm. Their findings indicate that SER-DT's performance is on par with that of CART, while simultaneously enhancing the model's explainability. This explainability is primarily achieved through the imposition of limitations on tree depth and the use of a minimal set of features in the decision-making rules. The model's explainability assumes significance in this context, as it has the potential to offer valuable insights into the decision-making strategies adopted by case workers when handling resource allocations. This resonates closely with Lipsky's assertion that caseworkers frequently employ heuristic methods to streamline their workload.

%R4's concerns about potential variability in tree-generated outputs align with SER-DT's design, allowing for slight variations in tree structures. However, we wish to reassure the reviewers that we have addressed this issue. We have computed average AUC scores from 10 different models, selecting the ones with the highest test accuracy for final predictions. Additionally, to mitigate concerns regarding model prediction discrepancies, we present Spearman's Rank Correlation in  and will include this in the final version of the paper as well. The heatmap in the figure 



%The thing about model 10 for ES is that its the worst performing model in terms of what SER-DT is optimizing for i.e. "Explanation Size". Model 10's is 3.12 compared to the average of 2.43 average of the other 9 models. In fact, this was the WORST performing in this regard in ALL the models we ever trained. The average explanation size of the SER-DT models we look at (minus model 10 for ES) is 2.11 with the maximum being 2.8. 

%We would like to express our sincere gratitude to the reviewers for their invaluable time and expertise. We have diligently and comprehensively attended to all the concerns raised, and as a result, we maintain a high degree of confidence in the robustness, validity, and significancee of our research findings.



% \newpage

% \textcolor{blue}{Reviewer 1 concerns: }

% \begin{itemize}
%     \item It seems likely that there could be many simple decision trees that have similar predictive accuracy. Have the authors studied this, and is there any way to show that a simple description of human decisions is well-identified?

%     \item Second, using BART estimates (or any similar method) relies on an assumption of no unobserved confounding. While many relevant variables are measured, this seems difficult to fully justify. This may be particularly consequential because the paper is precisely studying the impact of human discretion, where humans make decisions that deviate in some way from what Is expected, and the concern is always that human decision-makers do so based on features that are unobservable in the dataset, eg interactions with the clients. At the very least, it would be helpful to have more information about the setting — what opportunities are there for decision-makers to obtain this kind of information which is not present in the observed covariates? Further, is this concern mitigated by the high AUC of nonparametric models in fitting the decisions?

%     \item A more minor comment: it would be good to have confidence intervals for the AUCs, and to list in the main text what the sample size is.
% \end{itemize}


% \textcolor{blue}{Reviewer 3 concerns: }

% \begin{itemize}
%     \item How does the learned decision tree from other models (i.e. optimal trees, CART, etc.) differ from the SER-DT model used in this paper? Do these other ways of creating trees change the analysis?
    
%     \item Is there any insight into how close the estimation of the vulnerability score is to the actual scores that would be given by the VI-SPDAT? Are there any factors considered in the VI-SPDAT that could not be captured in the estimation of the vulnerability score?
% \end{itemize}



% \textcolor{blue}{Reviewer 4 concerns: }

% \begin{itemize}
%     \item \textbf{Scope and promise for social impact}: While the empirical findings seem quite interesting, I am unclear about the implications of this work from the get-go. If case worker behavior is highly predictable, wouldn’t this mean that they should be replaced by automated systems? I am very concerned about any conclusions like that.
%     \item[] 

%     \item \textbf{Justification of the approach}: I am unclear as to why the authors state that inconsistent application of discretionary power by caseworkers is necessarily problematic. Could it not just be that there are certain unobservables at play that justify human discretion in the first place? If decisions were to be always consistent, then why wouldn’t we just automate them and keep the human out of the loop? Again, I am concerned about any suggestions like that.
%     \item Why are the authors using (shallow) decision trees as interpretable models? Using these models to draw conclusions about behavior seems not valid.
%     \item The (implicitly assumed) relationship between inherently interpretable ML models and being able to infer human decision-making patterns is not clear to me and likely flawed. Statements like this, “As can be seen, the short rules are good at explaining a chunk of human decision-making regarding intervention assignments based on household characteristics” are entirely unclear to me. What is meant by “are good at explaining”? It seems that the authors are assuming the decision trees are equivalent to the human decision-making behavior (for the instances that the trees predict correctly?). But what about unobservables? What about features the trees are not considering?
%     \item[] 

%     \item \textbf{Quality of evaluation}: In line with what I said earlier, I am a concerned about the conclusions of this work: the authors conclude from the fact that caseworker decisions can be predicted well that their decisions are consistent. This conclusion is not obvious to me and seems to rest on some unstated (and perhaps wrong) assumptions. I’d want to see a more thorough justification of any such inferences.
%     \item Similarly for the conclusion on the application of discretion: why are these the cases that decision trees are not predicting correctly? There seems to be something missing in the argumentation here. What if cases are predicted correctly by some decision trees but not by others?
%     \item The authors seem to not have computed any confidence intervals and/or cross validation in their analyses.

%     \item[]

%     \item \textbf{Reproducibility and facilitation of follow-up work}: The authors make no reference to the data set they are working with. I don’t know how this data was obtained. This hampers reproducibility and follow-up work.

% \end{itemize}

==> feature_coeffs.tex <==
\newpage
\section{Appendix B}

\begin{table}[H]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|lcccc|}
\hline
\multicolumn{5}{|c|}{\textbf{Features Used to Predict Emergency Shelter}}                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{\textbf{Features}}                                                            & \multicolumn{1}{c|}{\textbf{Odds Ratio}} & \multicolumn{1}{c|}{\textbf{Lower CI}} & \multicolumn{1}{c|}{\textbf{Upper CI}} & \textbf{Ratio Satisfying} \\ \hline
\multicolumn{1}{|l|}{Gender Female}                                                                & \multicolumn{1}{c|}{8.91}                & \multicolumn{1}{c|}{8.88}              & \multicolumn{1}{c|}{8.95}              & 0.65                      \\ \hline
\multicolumn{1}{|l|}{Prior residence is Substance abuse treatment facility or detox center}        & \multicolumn{1}{c|}{1.85}                & \multicolumn{1}{c|}{1.84}              & \multicolumn{1}{c|}{1.86}              & 0.084                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Transitional housing for homeless persons}                 & \multicolumn{1}{c|}{1.74}                & \multicolumn{1}{c|}{1.73}              & \multicolumn{1}{c|}{1.75}              & 0.068                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Client refused}                                            & \multicolumn{1}{c|}{1.69}                & \multicolumn{1}{c|}{1.68}              & \multicolumn{1}{c|}{1.7}               & 0.063                     \\ \hline
\multicolumn{1}{|l|}{Primary race is White}                                                        & \multicolumn{1}{c|}{1.22}                & \multicolumn{1}{c|}{1.22}              & \multicolumn{1}{c|}{1.22}              & 0.151                     \\ \hline
\multicolumn{1}{|l|}{Calls}                                                                        & \multicolumn{1}{c|}{1.05}                & \multicolumn{1}{c|}{1.05}              & \multicolumn{1}{c|}{1.05}              &                           \\ \hline
\multicolumn{1}{|l|}{Children6\_10}                                                                & \multicolumn{1}{c|}{1.05}                & \multicolumn{1}{c|}{1.05}              & \multicolumn{1}{c|}{1.06}              &                           \\ \hline
\multicolumn{1}{|l|}{HasSubstanceAbuseProblem}                                                     & \multicolumn{1}{c|}{1.03}                & \multicolumn{1}{c|}{1.03}              & \multicolumn{1}{c|}{1.03}              & 0.065                     \\ \hline
\multicolumn{1}{|l|}{ReceivePhysicalDisabilityServices}                                            & \multicolumn{1}{c|}{1.02}                & \multicolumn{1}{c|}{1.02}              & \multicolumn{1}{c|}{1.02}              & 0.042                     \\ \hline
\multicolumn{1}{|l|}{Age}                                                                          & \multicolumn{1}{c|}{1.01}                & \multicolumn{1}{c|}{1.01}              & \multicolumn{1}{c|}{1.01}              &                           \\ \hline
\multicolumn{1}{|l|}{RatioOfNumCallstoWaitTime}                                                    & \multicolumn{1}{c|}{1}                   & \multicolumn{1}{c|}{1}                 & \multicolumn{1}{c|}{1}                 &                           \\ \hline
\multicolumn{1}{|l|}{MonthlyAmount}                                                                & \multicolumn{1}{c|}{1}                   & \multicolumn{1}{c|}{1}                 & \multicolumn{1}{c|}{1}                 &                           \\ \hline
\multicolumn{1}{|l|}{Wait}                                                                         & \multicolumn{1}{c|}{1}                   & \multicolumn{1}{c|}{1}                 & \multicolumn{1}{c|}{1}                 &                           \\ \hline
\multicolumn{1}{|l|}{Children}                                                                     & \multicolumn{1}{c|}{0.96}                & \multicolumn{1}{c|}{0.96}              & \multicolumn{1}{c|}{0.961}             &                           \\ \hline
\multicolumn{1}{|l|}{ReceiveChronicHealthServices}                                                 & \multicolumn{1}{c|}{0.932}               & \multicolumn{1}{c|}{0.931}             & \multicolumn{1}{c|}{0.933}             & 0.086                     \\ \hline
\multicolumn{1}{|l|}{Has a DisablingCondition}                                                     & \multicolumn{1}{c|}{0.903}               & \multicolumn{1}{c|}{0.902}             & \multicolumn{1}{c|}{0.905}             & 0.126                     \\ \hline
\multicolumn{1}{|l|}{HasChronicHealthCondition}                                                    & \multicolumn{1}{c|}{0.868}               & \multicolumn{1}{c|}{0.865}             & \multicolumn{1}{c|}{0.87}              & 0.188                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Staying or living in a family members room}                & \multicolumn{1}{c|}{0.67}                & \multicolumn{1}{c|}{0.663}             & \multicolumn{1}{c|}{0.676}             & 0.125                     \\ \hline
\multicolumn{1}{|l|}{Children15\_17}                                                               & \multicolumn{1}{c|}{0.551}               & \multicolumn{1}{c|}{0.541}             & \multicolumn{1}{c|}{0.56}              &                           \\ \hline
\multicolumn{1}{|l|}{ReceiveSubstanceAbuseServices}                                                & \multicolumn{1}{c|}{0.459}               & \multicolumn{1}{c|}{0.446}             & \multicolumn{1}{c|}{0.471}             & 0.072                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Staying or living in a friends room}                       & \multicolumn{1}{c|}{0.101}               & \multicolumn{1}{c|}{0.0649}            & \multicolumn{1}{c|}{0.137}             & 0.035                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Place not meant for habitation}                            & \multicolumn{1}{c|}{0.0768}              & \multicolumn{1}{c|}{0.0361}            & \multicolumn{1}{c|}{0.117}             & 0.053                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Client doesnt know}                                        & \multicolumn{1}{c|}{0.0349}              & \multicolumn{1}{c|}{-0.0183}           & \multicolumn{1}{c|}{0.088}             & 0.023                     \\ \hline
\multicolumn{1}{|l|}{HUDChronicHomeless}                                                           & \multicolumn{1}{c|}{0.0334}              & \multicolumn{1}{c|}{-0.0204}           & \multicolumn{1}{c|}{0.0872}            & 0.002                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Rental by client, with other ongoing housing subsidy}      & \multicolumn{1}{c|}{0.0269}              & \multicolumn{1}{c|}{-0.0304}           & \multicolumn{1}{c|}{0.0841}            & 0.016                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Rental by client, no ongoing housing subsidy}              & \multicolumn{1}{c|}{0.00304}             & \multicolumn{1}{c|}{-0.0887}           & \multicolumn{1}{c|}{0.0948}            & 0.197                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Owned by client, no ongoing housing subsidy}               & \multicolumn{1}{c|}{0.00257}             & \multicolumn{1}{c|}{-0.0918}           & \multicolumn{1}{c|}{0.097}             & 0.121                     \\ \hline
\multicolumn{5}{|c|}{\textbf{Features Used to Predict Transitional Housing}}                                                                                                                                                                                \\ \hline
\multicolumn{1}{|l|}{\textbf{Features}}                                                            & \multicolumn{1}{c|}{\textbf{Odds Ratio}} & \multicolumn{1}{c|}{\textbf{Lower CI}} & \multicolumn{1}{c|}{\textbf{Upper CI}} & \textbf{Ratio Satisfying} \\ \hline
\multicolumn{1}{|l|}{Gender Male}                                                                  & \multicolumn{1}{c|}{11.4}                & \multicolumn{1}{c|}{11.3}              & \multicolumn{1}{c|}{11.6}              & 0.35                      \\ \hline
\multicolumn{1}{|l|}{Prior residence is Client doesnt know}                                        & \multicolumn{1}{c|}{7.21}                & \multicolumn{1}{c|}{7.07}              & \multicolumn{1}{c|}{7.35}              & 0.023                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Place not meant for habitation}                            & \multicolumn{1}{c|}{3.13}                & \multicolumn{1}{c|}{3.05}              & \multicolumn{1}{c|}{3.21}              & 0.053                     \\ \hline
\multicolumn{1}{|l|}{ReceiveSubstanceAbuseServices}                                                & \multicolumn{1}{c|}{2.29}                & \multicolumn{1}{c|}{2.24}              & \multicolumn{1}{c|}{2.35}              & 0.072                     \\ \hline
\multicolumn{1}{|l|}{HUDChronicHomeless}                                                           & \multicolumn{1}{c|}{2.2}                 & \multicolumn{1}{c|}{2.14}              & \multicolumn{1}{c|}{2.25}              & 0.002                     \\ \hline
\multicolumn{1}{|l|}{Children0\_2}                                                                 & \multicolumn{1}{c|}{2.18}                & \multicolumn{1}{c|}{2.12}              & \multicolumn{1}{c|}{2.23}              &                           \\ \hline
\multicolumn{1}{|l|}{Prior residence is Other}                                                     & \multicolumn{1}{c|}{2.1}                 & \multicolumn{1}{c|}{2.05}              & \multicolumn{1}{c|}{2.16}              & 0.031                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Staying or living in a friends room}                       & \multicolumn{1}{c|}{1.81}                & \multicolumn{1}{c|}{1.77}              & \multicolumn{1}{c|}{1.85}              & 0.035                     \\ \hline
\multicolumn{1}{|l|}{Children}                                                                     & \multicolumn{1}{c|}{1.42}                & \multicolumn{1}{c|}{1.39}              & \multicolumn{1}{c|}{1.44}              &                           \\ \hline
\multicolumn{1}{|l|}{Client does not have PhysicalDisability}                                      & \multicolumn{1}{c|}{1.37}                & \multicolumn{1}{c|}{1.35}              & \multicolumn{1}{c|}{1.39}              & 0.88                      \\ \hline
\multicolumn{1}{|l|}{Prior residence is Client refused}                                            & \multicolumn{1}{c|}{1.36}                & \multicolumn{1}{c|}{1.34}              & \multicolumn{1}{c|}{1.38}              & 0.063                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Hotel or motel paid for without emergency shelter voucher} & \multicolumn{1}{c|}{1.36}                & \multicolumn{1}{c|}{1.34}              & \multicolumn{1}{c|}{1.38}              & 0.007                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Emergency shelter}                                         & \multicolumn{1}{c|}{1.35}                & \multicolumn{1}{c|}{1.33}              & \multicolumn{1}{c|}{1.37}              & 0.133                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Staying or living in a family members room}                & \multicolumn{1}{c|}{1.26}                & \multicolumn{1}{c|}{1.25}              & \multicolumn{1}{c|}{1.28}              & 0.125                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Substance abuse treatment facility or detox center}        & \multicolumn{1}{c|}{1.25}                & \multicolumn{1}{c|}{1.24}              & \multicolumn{1}{c|}{1.27}              & 0.084                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Transitional housing for homeless persons}                 & \multicolumn{1}{c|}{1.1}                 & \multicolumn{1}{c|}{1.09}              & \multicolumn{1}{c|}{1.11}              & 0.068                     \\ \hline
\multicolumn{1}{|l|}{Primary race is Black}                                                        & \multicolumn{1}{c|}{1.04}                & \multicolumn{1}{c|}{1.04}              & \multicolumn{1}{c|}{1.05}              & 0.833                     \\ \hline
\multicolumn{1}{|l|}{Calls}                                                                        & \multicolumn{1}{c|}{1.02}                & \multicolumn{1}{c|}{1.01}              & \multicolumn{1}{c|}{1.02}              &                           \\ \hline
\multicolumn{1}{|l|}{RatioOfNumCallstoWaitTime}                                                    & \multicolumn{1}{c|}{1.01}                & \multicolumn{1}{c|}{1.01}              & \multicolumn{1}{c|}{1.01}              &                           \\ \hline
\multicolumn{1}{|l|}{Wait}                                                                         & \multicolumn{1}{c|}{1}                   & \multicolumn{1}{c|}{1}                 & \multicolumn{1}{c|}{1}                 &                           \\ \hline
\multicolumn{1}{|l|}{MonthlyAmount}                                                                & \multicolumn{1}{c|}{0.999}               & \multicolumn{1}{c|}{0.999}             & \multicolumn{1}{c|}{0.999}             &                           \\ \hline
\multicolumn{1}{|l|}{Age}                                                                          & \multicolumn{1}{c|}{0.969}               & \multicolumn{1}{c|}{0.967}             & \multicolumn{1}{c|}{0.971}             &                           \\ \hline
\multicolumn{1}{|l|}{Primary race is White}                                                        & \multicolumn{1}{c|}{0.853}               & \multicolumn{1}{c|}{0.842}             & \multicolumn{1}{c|}{0.864}             & 0.151                     \\ \hline
\multicolumn{1}{|l|}{HasMentalHealthProblem}                                                       & \multicolumn{1}{c|}{0.611}               & \multicolumn{1}{c|}{0.576}             & \multicolumn{1}{c|}{0.645}             & 0.185                     \\ \hline
\multicolumn{1}{|l|}{num\_members}                                                                 & \multicolumn{1}{c|}{0.485}               & \multicolumn{1}{c|}{0.434}             & \multicolumn{1}{c|}{0.536}             &                           \\ \hline
\multicolumn{1}{|l|}{SpousePresent}                                                                & \multicolumn{1}{c|}{0.344}               & \multicolumn{1}{c|}{0.269}             & \multicolumn{1}{c|}{0.419}             & 0.004                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Owned by client, no ongoing housing subsidy}               & \multicolumn{1}{c|}{0.105}               & \multicolumn{1}{c|}{-0.053}            & \multicolumn{1}{c|}{0.264}             & 0.121                     \\ \hline
\multicolumn{1}{|l|}{Prior residence is Rental by client, no ongoing housing subsidy}              & \multicolumn{1}{c|}{0.0811}              & \multicolumn{1}{c|}{-0.0955}           & \multicolumn{1}{c|}{0.258}             & 0.197                     \\ \hline
\end{tabular}%
}
\end{table}

==> introduction-old.tex <==
\section{Introduction}

Homelessness is an acute and pervasive issue affecting societies worldwide. The lack of stable housing and access to resources poses immense challenges for individuals and families, jeopardizing their well-being and livelihoods. In the United States, the coordination of homeless services at the community level, encounters significant challenges in meeting the overwhelming demand for housing assistance. Regrettably, there is limited evidence available to substantiate the accuracy of current decision-making practices in allocating the scarce resources within the realm of homeless services \cite{ VISPDAT_validity, capability_traps, efficient_targeting_shinn}. However, recent advancements in machine learning (ML) and artificial intelligence (AI) techniques have presented opportunities to apply learning algorithms to address social issues spanning various domains, including law enforcement and wildlife conservation. These innovative solutions have demonstrated successful outcomes in mitigating the specific problems to which they were applied \cite{Carthy_Vayanos_Tambe_2017,optimal_alloc_cts_time}. Even within the realm of homelessness services, ML models have emerged as valuable tools for addressing the challenge of predicting outcomes of interventions for households at risk of homelessness \cite{Kube_Das_Fowler_2019}. 

As federal guidelines increasingly emphasize entirely alleviating homelessness \cite{all_in_2022}, a need exists for not only a comprehensive understanding of its causes and dynamics but also the strategic allocation of limited resources to provide timely interventions. In this study, we utilize the pattern recognition capabilities of ML models to forecast the interventions that households are likely to receive upon entering the homeless system. 



\subsubsection{Ethics and Fairness:} When addressing the allocation of scarce societal resources through algorithmic approaches, it is imperative to prioritize discussions on ethical issues and fairness. The widespread use of AI and machine learning in society has raised concerns about accountability and transparency \cite{Neil_2016}, as data-driven allocations can perpetuate biases and inequities \cite{ensign_2017, pleiss_2017, Corbet_2017}. The complexity of developing decision algorithms has cast doubts on the ability to design adequate protections against systematic misuses. Responding to these concerns, the European Union has introduced the ``General Data Protection Regulation’’ (GDPR), imposing limitations on individual data utilization for algorithmic decision-making processes with a ``significant effect" on users. The GDPR aligns with a broader argument emphasizing the importance of not only full transparency but also human interpretability to comprehend how decisions arise from algorithmic approaches.

The call for interpretability aims to assess fairness thoroughly. \citet{Doshi_Kim_2017} highlight the importance of interpretable machine learning and advocate for a scientific approach to advance the field. Explainable AI enables human understanding of algorithmic outputs, empowering caseworkers to validate predictions against their domain knowledge and professional judgment, fostering trust and fairness in resource allocation. In a critical infrastructure like the homelessness system, predicting intervention assignments using explainable AI could provide interpretable explanations, such as feature importance and decision rules, assisting caseworkers in comprehending model rationale. In an effort to explain model characteristics, several techniques like the LIME framework \cite{LIME}, SHAP values \cite{SHAP}, and risk scores \cite{rudin_2019} have been used in the field. But the use of such black-box, model-independent metrics, while offering valuable insights into opaque models, suffer from limitations. Firstly, their model-agnostic nature may lead to explanations that fail to capture the idiosyncrasies of specific models, potentially compromising the accuracy of the interpretations. Additionally, the computational overhead required for implementing SHAP and LIME can be substantial. In this study, we embrace Decision Trees (DT) as the model of choice due to their inherent interpretable nature, the importance of which has been stressed by \citet{rudin_2019} when making high-stakes decisions. DTs' model-specificity ensures accurate representations of individual models, providing clear insights into feature contributions and decision rules. To further enhance interpretability, we also incorporate a recent algorithmic technique proposed by \citet{SERDT} to make the DTs shorter and more interpretable. Explainable AI provides transparency and interpretability, allowing stakeholders, including caseworkers, policymakers, and individuals affected by homelessness, to comprehend the decision-making process and have confidence in the outcomes.



\subsubsection{Resource allocation for social services:}

\subsubsection{Problem Setup}
In the United States, local homeless systems coordinate a range of interventions to address housing crises, spanning from time-limited non-residential supports to ongoing rental assistance with intensive case management \cite{HEARTH2009}. The demand for affordable housing remains constant and widespread, leading to capacity constraints in each service, presenting homeless providers with the challenging task of allocating households to available interventions. In such a situation, precise prediction of the interventions households might receive becomes crucial in optimizing resource allocation strategies and enhancing the effectiveness of homeless services, enabling timely and targeted assistance, and reducing re-entry rates within the homeless system. Policymakers, caseworkers, and service providers can leverage this accurate prediction to make informed decisions, promoting transparency and accountability in addressing homelessness.

To accomplish this, we utilize unique local administrative records, linking homeless service records with requests for assistance through a regional homeless hotline. This comprehensive data collection surpasses federal requirements and facilitates a thorough assessment of homeless services, making it possible to predict interventions with decision trees (DTs). More specifically, we employ two algorithms: the standard Classification and Regression Trees (CART) and the Short Explainable Rules - Decision Tree (SER-DT) \cite{SERDT}, which prioritizes interpretability by optimizing "explanation size." Results indicate that our models can accurately predict intervention assignments, but they are not infallible and are sometimes wrong. In cases where the models make errors, we hypothesize that caseworker discretion is being applied which we try to characterize in this study. By characterizing discretionary choices exhibited by caseworkers in assigning interventions, we aim to uncover the factors and considerations guiding deviations from rule-based predictions. Explainable AI, in this context, can provide valuable insights into the nuanced judgment and intuition caseworkers bring to the decision-making process.


\subsubsection{Preview of Results} Our implemented models demonstrate remarkable accuracy in predicting interventions, as indicated by high Area Under the Curve (AUC) values. Specifically, the AUC values for Emergency Shelter (ES), Transitional Housing (TH), Rapid Rehousing (RRH), and Prevention (Prev) interventions are 0.91, 0.92, 0.83, and 0.97, respectively. These results affirm the model's overall proficiency in predicting interventions, yet it exhibits varying predictive performance across different intervention types. Interestingly, we observed that the decision tree rules generated by the models tend to be highly complex despite their high accuracy rates. However, simplifying these rules while maintaining satisfactory performance highlights that a considerable portion of the models' effectiveness can be explained by simple rules. Even when employing simple rules, the model continues to achieve notable AUC values of 0.73, 0.78, 0.53, and 0.90, respectively, for ES, TH, RRH, and Prev interventions. Yet, the question arises: what happens when the models make errors? Our hypothesis suggests that these errors may stem from caseworkers exercising discretion in their decision-making process. Our results show that, when considering ES and TH as two interventions with varying levels of intensity, when caseworkers deviate from the rules, it results in improved outcomes for households receiving interventions.

\subsubsection{Implications} Our results indicate that when caseworkers employ discretionary behavior, the outcomes consistently exhibit superior quality.  Accurately identifying and quantifying the discretionary choices made by caseworkers when assigning interventions to households seeking federal homelessness services holds immense potential in terms of the design and implementation of new systems. This information can be utilized to develop targeted training programs aimed at equipping caseworkers with the requisite knowledge and skills to make informed decisions and achieve positive, sustainable outcomes for homeless households.

 Moreover, such quantification represents a critical initial step toward establishing a framework that ensures justice and consistency in the allocation of vital resources. By gaining a deeper understanding of how organizational policies interact with the street-level bureaucracy \cite{Lipsky_2010} typically employed by caseworkers, we can foster greater clarity and transparency in resource distribution processes. Consequently, this framework promotes a comprehensive comprehension of the intricate dynamics between organizational policies and the caseworkers responsible for implementing them.






% In recent years, machine learning (ML) models have emerged as valuable tools for addressing the challenge of predicting outcomes of interventions for households at risk of homelessness \cite{JAIR,Kube_Das_Fowler_2019,JAMIA}. In this study, we utilize the pattern recognition capabilities of ML models to forecast the interventions that households are likely to receive upon entering the homeless system. By adopting an explainable AI approach, these models provide insights into the assignment process for specific intervention types. Our implementation of these models demonstrates impressive accuracy in predicting interventions and has achieved high Area Under the Curve (AUC) values. However, an interesting observation arises from our findings: the decision tree rules generated by the models tend to be highly intricate, given their high accuracy rates. Simplifying these rules while maintaining satisfactory performance reveals that much of the models' effectiveness can be explained by simple rules. So how about when the models are wrong? We hypothesize that such errors occur when caseworkers exercise discretion in their decision-making process. Caseworkers, guided by their intuition and judgment, often deviate from the rules, leading to improved outcomes
% {\color{red}[is this a citation or one of our results?]}.

% Our results indicate that when caseworkers employ discretionary behavior, the outcomes consistently exhibit superior quality. Therefore, comprehending this discretionary behavior is crucial for optimizing resource allocation strategies and ensuring equitable outcomes. Accurately identifying and quantifying the discretionary choices made by caseworkers when assigning interventions to households seeking federal homelessness services holds immense potential to bring about transformative impacts on the lives of individuals in need. This valuable information can be utilized to develop targeted training programs aimed at equipping caseworkers with the requisite knowledge and skills to make informed decisions and achieve positive, sustainable outcomes for homeless households.

% Moreover, such quantification represents a critical initial step toward establishing a framework that ensures justice and consistency in the allocation of vital resources. By gaining a deeper understanding of how organizational policies interact with the street-level bureaucracy \cite{Lipsky_2010} typically employed by caseworkers, we can foster greater clarity and transparency in resource distribution processes. Consequently, this framework promotes a comprehensive comprehension of the intricate dynamics between organizational policies and the caseworkers responsible for implementing them.



% The coordination of homeless services at the community level, within the broader homeless system, encounters significant challenges in meeting the overwhelming demand for housing assistance. Regrettably, there is limited evidence available to substantiate the accuracy of current decision-making practices in allocating the scarce resources within the realm of homeless services \cite{ VISPDAT_validity, capability_traps, efficient_targeting_shinn}. However, recent advancements in machine learning and artificial intelligence (AI) techniques have presented opportunities to apply learning algorithms to address social issues spanning various domains, including law enforcement and wildlife conservation. These innovative solutions have demonstrated successful outcomes in mitigating the specific problems to which they were applied \cite{Carthy_Vayanos_Tambe_2017,optimal_alloc_cts_time}.

==> papers_citing_lipsky.tex <==


% \begin{itemize}
%     \item \textbf{What to account for when accounting for algorithms \cite{accountability_wieringa2020}: } This paper presents a systematic literature review on algorithmic accountability, emphasizing the need for a comprehensive accountability relationship that encompasses the entire socio-technical process of algorithmic systems. The term ``algorithmic accountability" is defined as a networked account involving multiple actors throughout the system's life-cycle. These actors, such as decision makers, developers, and users, have the obligation to explain and justify their actions concerning the system and its effects. The review identifies five essential elements: actors, fora, perspective, account, and consequences. The paper emphasizes the importance of balancing these elements to achieve effective accountability. It also highlights the need for interdisciplinary engagement, considering the perspectives from various domains where algorithmic systems are applied. The study suggests that accountability theory from governance studies should be more widely referenced. Future research is encouraged to ground accountability theory and explore the discrepancies between different fields' perspectives on algorithmic accountability. Overall, the paper calls for a holistic approach in addressing the challenges of holding algorithmic systems accountable.


%     \item \textbf{Improving Human-AI Partnerships in Child Welfare: Understanding Worker Practices, Challenges, and Desires for Algorithmic Decision Support \cite{childWelfare2022}}: This paper conducts a detailed qualitative investigation into how child welfare workers utilize an AI Decision Support system called the Allegheny Family Screening Tool (AFST) in their day-to-day decision-making processes. The AFST is designed to predict longer-term risk and adverse outcomes over a two-year time-span, complementing workers' immediate safety and short-term risk focus. However, the study finds that workers often perceive value misalignments between the ADS's predictive targets and their own decision objectives. Some workers are open to the idea of the AFST complementing their judgment and mitigating biases, but others disagree with making screening decisions based on longer-term risk predictions, seeing it as fundamentally misaligned with their roles and responsibilities. Despite using the AFST for a considerable period, workers received minimal training and had little formal insight into how the system works. They compensated for the limitations of the ADS by relying on their rich contextual knowledge of individual cases, engaging in collective sensemaking and decision-making among themselves. Organizational pressures and incentives also influenced workers' reliance on the ADS, sometimes leading them to comply with the AFST's recommendation even against their best judgment. Additionally, workers felt they had limited agency in shaping the ADS's use or improving its accuracy. The paper highlights the need to address human-AI value misalignments, provide better training and transparency about the system's capabilities, foster open discussions, and involve diverse stakeholders in the design process. The aim is to support human-AI complementarity and enhance decision-making in child welfare and other public sector contexts effectively.



%     \item{\textbf{Understanding Frontline Workers’ and Unhoused Individuals’ Perspectives on AI Used in Homeless Services} \cite{homelessnesPerspective2023}}  The authors conducted an in-depth study using AI lifecycle comicboarding, a novel method that allowed frontline workers and unhoused individuals to provide specific feedback on the AI system's design and deployment. One crucial finding was that non-AI experts can offer valuable insights into AI systems, challenging the common skepticism that only AI experts can provide meaningful feedback. Participants expressed concerns about potential biases and harm caused by the algorithm, particularly in its optimization towards the county's interests rather than addressing the needs and safety of unhoused individuals. They also raised doubts about the validity and reliability of certain aspects of the model's design, such as the use of proxy variables for real-world outcomes. Participants offered alternative ways to use the data available to the county for service provision, proposing a system that actively connects individuals with various resources based on their specific needs. They also emphasized the importance of downstream care plans customized for each individual to prevent them from cycling back to homelessness. Moreover, the study highlighted the need for more upfront work to connect people to AI systems and emphasized the value of qualitative narratives in complementing quantitative data for decision-making.

%     The paper underscores the significance of incorporating diverse perspectives and empowering frontline workers in the AI system design process. By using AI lifecycle comicboarding early in the design stages, developers can effectively integrate feedback and make meaningful changes to address potential harm and biases. This approach can improve the ethical and practical implications of AI systems, ensuring they better serve the marginalized and vulnerable populations they are designed to support. The study lays the foundation for future research to adapt the comicboarding method for other disadvantaged groups, fostering a more inclusive and participatory approach to AI system design across various social challenges.
    
% \end{itemize}
